Semantic Scene Completion using Local Deep Implicit Functions on LiDAR Data

Semantic scene completion is the task of jointly estimating 3D geometry and semantics of objects and surfaces within a given extent. This is a particularly challenging task on real-world data that is sparse and occluded. We propose a scene segmentation network based on local Deep Implicit Functions as a novel learning-based method for scene completion. Unlike previous work on scene completion, our method produces a continuous scene representation that is not based on voxelization. We encode raw point clouds into a latent space locally and at multiple spatial resolutions. A global scene completion function is subsequently assembled from the localized function patches. We show that this continuous representation is suitable to encode geometric and semantic properties of extensive outdoor scenes without the need for spatial discretization (thus avoiding the trade-off between level of scene detail and the scene extent that can be covered). We train and evaluate our method on semantically annotated LiDAR scans from the Semantic KITTI dataset. Our experiments verify that our method generates a powerful representation that can be decoded into a dense 3D description of a given scene. The performance of our method surpasses the state of the art on the Semantic KITTI Scene Completion Benchmark in terms of geometric completion intersection-over-union (IoU).

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> figures/figure_dataset.tex <==
% !TEX root = ../root.tex
%%
\begin{figure}[t]
    \centering{}
    \renewcommand{\arraystretch}{0.3} % vertical spacing between rows
    \setlength{\tabcolsep}{1pt} % horizontal spacing between columns
    
    \begin{tabularx}{\linewidth}{XX}
        \includegraphics[width=\linewidth]%
        {media/fig_dataset/semantic_kitti_00_0000_sparse.png_converted.jpg} &
        \includegraphics[width=\linewidth]%
        {media/fig_dataset/semantic_kitti_00_0000_dense.png_converted.jpg} \\
        \subfloat[Input: Single LiDAR point cloud]{\includegraphics[width=\linewidth]%
        {media/fig_dataset/semantic_kitti_08_0000_sparse.png_converted.jpg}%
        \label{fig:dataset_single}} &
        \subfloat[Target: Accumulated point clouds]{\includegraphics[width=\linewidth]%
        {media/fig_dataset/semantic_kitti_08_0000_dense.png_converted.jpg}%
        \label{fig:dataset_accumulated}} \\
    \end{tabularx}
    %
    \caption{%
    \textbf{Accumulation of LiDAR measurements for the scene completion task:}
    The left column \protect\subref{fig:dataset_single} shows the single LiDAR sweep
    which serves as the input to the scene completion method (without semantic
    annotations).
    The right column \protect\subref{fig:dataset_accumulated} shows the accumulated
    LiDAR measurements with semantic annotations that are used as training targets
    for scene completion.
    The point of view is the (invisible) ego-vehicle on the center-left position
    in the images.
    All dynamic objects (cars, bicycles, motorbikes on road and pedestrians) consist
    only of the single LiDAR sweep from the view-point of the ego-vehicle.
    The black areas in \protect\subref{fig:dataset_accumulated} are shadows from
    this view-point that are cast by dynamic objects.
    The training loss is omitted in these occluded areas to allow the network to predict a static scene that is geometrically consistent.%
    \label{fig:dataset}%
    }

\end{figure}


==> figures/figure_latent_grid.tex <==
% !TEX root = ../root.tex
%%
\begin{figure}[htb]
    \centering{}
    %
    \begin{tikzpicture}
        \node[anchor=south west,inner sep=0] (image) at (0,0) %
        {\includegraphics[width=.8\linewidth]{media/latent_grid_render.jpg}};
          \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw ({0.2}, {0.7}) node {\small{$c_1$, \SI{5.12}{\meter}}};
            \draw ({0.2}, {0.53}) node {\small{$c_2$, \SI{1.28}{\meter}}};
            \draw ({0.2}, {0.36}) node {\small{$c_3$, \SI{0.32}{\meter}}};
          \end{scope}
    \end{tikzpicture}
    %
    \caption{%
    Spatial structure of the three resolution feature maps $c_1$, $c_2$, $c_3$
    that make up the latent representation.
    Depiction of the ego-vehicle for scale.
    \label{fig:latent_grid}%
    }
%
\end{figure}

==> tables/table_validation_dataset_comp.tex <==
% !TEX root = ../root.tex
%%

\setlength{\tabcolsep}{4pt} % horizontal spacing between columns
\begin{table}[tb]
\caption{Training for scene completion vs. scan segmentation}
\label{tab:semantic_vs_completion}
\centering
%
\begin{tabularx}{\linewidth}{@{}lrr@{}}
\toprule
Training targets & \pbox{1.7cm}{Geometric Completion IoU} & \pbox{2cm}{Semantic Completion IoU} \\ \midrule
Static scene & 53.82 & 22.89 \\
Spatio-temporal tubes & 53.82 & 21.27 \\ \bottomrule
\end{tabularx}
%
\end{table}
